PREEMPT: Proactive Robustness Evaluation under Editing for Media Protection Techniques

Proactive image protection methods aim to defend visual content against unauthorized manipulation and generative misuse by embedding protective signals into images before release. Evaluating whether these protections remain effective under image editing is therefore critical. However, existing evaluations remain largely limited to one-shot edits, providing only a static view of robustness while overlooking its evolution under realistic multi-step editing workflows. To systematically characterize robustness dynamics under sequential editing across various protection paradigms, we introduce PREEMPT, a holistic evaluation framework. It evaluates protection robustness under both one-shot and sequential editing scenarios, covering image transformations, semantic edits, homogeneous and heterogeneous edit compositions. To enable consistent analysis across protection paradigms with different underlying objectives, PREEMPT normalizes task-specific effectiveness into protection survival trajectories and summarizes long-horizon robustness through trajectory-based diagnostics. Using this framework, we reveal that degradation behaviors remain hidden under conventional one-shot evaluation. Furthermore, perturbation- and watermark-based protection methods exhibit different failure modes, and the first semantic edit largely determines subsequent degradation trajectories. PREEMPT provides a standardized protocol for studying long-horizon robustness and offers new insights into the degradation dynamics of proactive image protection.

==> round1/0_abstract.tex <==
\begin{abstract}
% Proactive image protection methods embed protective signals into images before release to safeguard visual content from unauthorized manipulation and generative misuse. Despite rapid progress in both adversarial perturbation and watermark-based approaches, robustness evaluation remains largely limited to isolated single-edit tests, providing only static endpoint measurements and failing to reflect realistic editing workflows involving diverse and repeated manipulations.
% In this paper, we present PREEMPT, an evaluation framework for analyzing the robustness dynamics of proactive image protection. Instead of assessing robustness based on the result of a single edit, our framework models protection effectiveness as a degradation process over edit type and editing depth. The framework consists of two complementary settings: One-Shot Edit, covering both image-transformation-based and semantic edits, and Sequential Edit, which evaluates progressive chains of homogeneous and heterogeneous edits. To make degradation comparable, PREEMPT reports three diagnostic metrics, Protection Survival Curve, Protection half-life and Protection AUC, to characterize robustness evolution throughout the editing process.
% Through extensive experiments across multiple visual domains and representative protection methods, we show that conventional single-edit evaluations can provide incomplete and sometimes misleading estimates of robustness. Different methods exhibit distinct degradation behaviors, and their relative effectiveness varies across editing depths and edit compositions. PREEMPT provides a systematic framework for diagnosing failure modes and guiding the development of future image protection methods with stronger long-term robustness.

% Proactive image protection methods embed protective signals into images before release to safeguard visual content from unauthorized manipulation and generative misuse. Despite rapid progress in both adversarial perturbation and watermark-based approaches, robustness evaluation remains largely limited to isolated single-edit tests, providing only static endpoint measurements and failing to reflect realistic editing workflows involving diverse and repeated manipulations.
Proactive image protection methods aim to defend visual content against unauthorized manipulation and generative misuse by embedding protective signals into images before release. Evaluating whether these protections remain effective under image editing is therefore critical. However, existing evaluations remain largely limited to one-shot edits, providing only a static view of robustness while overlooking its evolution under realistic multi-step editing workflows. To systematically characterize robustness dynamics under sequential editing across various protection paradigms, we introduce PREEMPT, a holistic evaluation framework. It evaluates protection robustness under both one-shot and sequential editing scenarios, covering image transformations, semantic edits, homogeneous and heterogeneous edit compositions. To enable consistent analysis across protection paradigms with different underlying objectives, PREEMPT normalizes task-specific effectiveness into protection survival trajectories and summarizes long-horizon robustness through trajectory-based diagnostics. Using this framework, we reveal that degradation behaviors remain hidden under conventional one-shot evaluation. We further find that perturbation- and watermark-based protection methods exhibit fundamentally different failure modes, and that the first semantic edit largely determines subsequent degradation trajectories. PREEMPT provides a standardized protocol for studying long-horizon robustness and offers new insights into the degradation dynamics of proactive image protection.

\end{abstract}


==> round1/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Motivation
% HOOK -> Background -> Threat -> Existing solutions
Recent advances in generative AI have made high-quality image editing increasingly accessible. Modern diffusion models~\cite{ho2020denoising, song2021denoising} enable realistic image manipulation~\cite{brooks2023instructpix2pix, couairon2022diffedit} and personalization~\cite{ruiz2023dreambooth, hu2022lora, gal2022image} from only a few user instructions, but these capabilities also raise concerns about unauthorized content modification, identity misuse, and style imitation. To mitigate such risks, proactive image protection methods~\cite{salman2023raising, jeong2025faceshield, tang2025styleprotect, wen2023treerings, fernandez2023stable} have been proposed to embed protective signals into images before release. Existing approaches mainly fall into two categories: perturbation-based methods~\cite{liu2024metacloak, shan2023glaze, xu2024perturbing}, which attempt to disrupt downstream generation behaviors, and watermark-based methods~\cite{liu2025watermarking, ye2024duaw, cui2025diffusionshield}, which enable ownership verification and content tracing after manipulation.

% Challenge and Gap
% Consequently, current evaluations~\cite{zhang2018unreasonable, hessel2021clipscore, heusel2017gans, xu2025lmm4edit} may substantially overestimate protection effectiveness and provide limited insight into how robustness degrades over time. The lack of a standardized and comprehensive evaluation framework also makes fair comparison across protection methods difficult.
% Despite the rapid progress of proactive image protection techniques, their robustness evaluation remains fragmented. 
% Existing studies often inherit experimental protocols from prior work, resulting in inconsistent choices of datasets, editing models, and evaluation criteria. Furthermore, robustness is typically assessed under isolated one-shot edits, whereas real-world image manipulations frequently involve multiple sequential operations whose cumulative effects remain largely unexplored. Another challenge arises from the method-specific nature of existing evaluations. Perturbation- and watermark-based methods are optimized for different objectives and therefore evaluated using different metrics, making direct comparison difficult. 
% Consequently, current evaluations may substantially overestimate protection effectiveness while providing limited insight into how protection sustains realistic editing workflows. 
% The lack of a standardized and comprehensive evaluation protocol also hinders fair comparison across protection paradigms.

Existing robustness evaluations~\cite{zhang2018unreasonable, hessel2021clipscore, heusel2017gans, xu2025lmm4edit} suffer from three major limitations. First, experimental protocols differ substantially across studies, with inconsistent choices of datasets, editing models, and evaluation criteria. Second, robustness is typically evaluated under isolated one-shot edits, while realistic image manipulations often involve multiple sequential operations whose cumulative effects remain poorly understood. Third, evaluations are method-specific: perturbation- and watermark-based methods are designed for different objectives and consequently rely on different performance metrics. Together, these limitations hinder fair comparison across protection methods and provide only a limited understanding of robustness under realistic edits.

% Fill the gap
To address these limitations, we introduce the \textbf{Pr}oactive \textbf{E}valuation under \textbf{E}diting for \textbf{M}edia \textbf{P}rotection \textbf{T}echniques, (\textbf{PREEMPT}), a robustness evaluation framework for proactive image protection. PREEMPT systematically evaluates protection methods under both one-shot and long-horizon sequential editing scenarios, covering homogeneous semantic chains and heterogeneous mixed editing workflows. To enable consistent analysis across heterogeneous protection paradigms, PREEMPT further introduces a trajectory-based robustness representation consisting of Protection Survival Ratio (PSR), Protection Survival Curves, and Protection AUC, which respectively provide a unified robustness representation, trajectory-level visualization, and compact robustness summarization across heterogeneous protection paradigms.


% Contributions
Our contributions are summarized as follows:

\begin{itemize}

\item We propose PREEMPT, the first unified robustness evaluation framework for proactive image protection, which systematically evaluates protection methods under both one-shot and long-horizon sequential editing scenarios.

\item We introduce a trajectory-based robustness characterization based on the Protection Survival Curves, together with Protection Survival Ratio (PSR) and Protection AUC, enabling consistent robustness analysis across perturbation- and watermark-based protection paradigms.

\item Using PREEMPT, we uncover several previously overlooked properties of proactive image protection, including continuous robustness evolution under sequential editing, paradigm-specific evolution patterns, ranking instability beyond one-shot evaluation, and the dominant role of semantic edits in long-horizon robustness.

\end{itemize}

% The remainder of this paper is organized as follows. Section~\ref{sec:related_work} reviews related work. Section~\ref{sec:method} presents PREEMPT. Sections~\ref{sec:one_shot_results} and~\ref{sec:sequential_result} evaluate one-shot and long-horizon robustness, respectively. Section~\ref{sec:conclusion} concludes the paper.

==> round1/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
% Fill the gap
\subsection{Proactive Image Protection}
% adversarial perturbation
%     PhotoGuard
%     Mist
%     Glaze
%     Anti-DreamBooth
%     AdvDM
% watermarking
%     WAM
%     StegaStamp
%     Tree-Ring
%     Stable Signature

Proactive image protection aims to safeguard visual assets before they are released by embedding protective signals into images, thereby preventing unauthorized editing, personalization, or redistribution. Existing approaches can be broadly categorized into \emph{watermark-based} and \emph{perturbation-based} methods, which differ in both their protection objectives and underlying mechanisms. 

Watermark-based methods~\cite{lu2024robust, lei2024diffusetrace, zhang2024editguard, liu2025watermarking} embed identifiable information into images for ownership attribution, authenticity verification, and provenance tracing. Traditional watermarking techniques have recently been extended to diffusion-based generative models. Representative approaches include StegaStamp~\cite{Tancik_2020_CVPR}, which embeds recoverable signatures for copyright verification, Tree-Ring Watermarks~\cite{wen2023treerings}, which inject structured patterns into diffusion latents for provenance tracing, Stable Signature~\cite{fernandez2023stable}, which integrates watermark generation into image synthesis, and WAM~\cite{sander2025watermark}, which improves watermark robustness against common image editing and post-processing operations. Rather than preventing manipulation itself, these methods aim to preserve the recoverability of embedded messages after image modifications. 

In contrast, perturbation-based methods~\cite{wang2024edit, shan2023glaze, mi2024visual, xue2023toward} proactively interfere with downstream image editing and model customization by introducing carefully optimized adversarial perturbations. 
% Representative methods include PhotoGuard~\cite{salman2023raising}, which disrupts the denoising process of diffusion models, Mist~\cite{liang2023mist}, which degrades editing quality through adversarial optimization, Glaze~\cite{shan2023glaze}, which prevents artistic style imitation, Anti-DreamBooth~\cite{van2023anti}, which targets personalization attacks, and AdvDM~\cite{liang2023adversarial}, which further improves protection effectiveness using diffusion-based adversarial optimization. 
Representative perturbation-based methods differ substantially in their protection mechanisms. PhotoGuard~\cite{salman2023raising} disrupts the diffusion inference pipeline through adversarial perturbations, whereas Glaze~\cite{shan2023glaze} protects artistic styles by shifting feature representations toward surrogate targets. To disrupt the generation quality, AdvDM~\cite{liang2023adversarial} further formulates perturbation generation directly using the diffusion objective, MIST~\cite{liang2023mist} improves perturbation transferability via semantic-aware adversarial optimization. For personalization mimicry, Anti-DreamBooth~\cite{van2023anti} explicitly optimizes against the dynamic fine-tuning process.
Unlike watermarking methods, perturbation-based ones seek to reduce the fidelity of downstream generation while remaining visually imperceptible. 

Although the two paradigms pursue different protection objectives~\cite{tang2025watermarks, tang2025perturbation}, both fundamentally rely on the persistence of embedded protective signals throughout subsequent editing operations. Their robustness is therefore determined not only by the protection algorithm itself but also by the editing process that follows image release. This shared dependency motivates the need for a unified robustness evaluation framework capable of consistently assessing heterogeneous protection paradigms under realistic editing workflows.

% \subsection{Image Editing Scenarios}

% Real-world images often experience multiple manipulations rather than a single isolated edit.

\subsection{Existing Robustness Evaluation}

Existing robustness evaluation protocols differ substantially across protection paradigms. Watermark-based methods~\cite{rabbani2024waves} typically assess robustness by measuring message retrieval accuracy or decoding success rate after image manipulations, with the objective of preserving watermark detectability throughout the editing process. Consequently, robustness is commonly evaluated under a collection of image transformations or semantic editing attacks by examining whether the embedded message can still be successfully recovered~\cite{lu2024robust}. 
Whereas, perturbation-based methods usually evaluate two complementary aspects: perturbation imperceptibility and protection effectiveness. Imperceptibility is measured using perceptual image quality metrics such as LPIPS~\cite{zhang2018unreasonable}, while protection effectiveness is typically quantified by applying a single semantic edit and measuring the semantic similarity between the edited result and the protected image.

Besides semantic edits, robustness against image transformations has become a standard component of protection evaluation. Common operations include JPEG compression, Gaussian blur, crop-and-resize, horizontal flipping, and brightness/contrast adjustment, which are widely adopted to simulate the automatic preprocessing pipelines applied by online social networks (OSNs) after image upload~\cite{liu2023generating}. Since adversarial perturbations are particularly vulnerable to these lossy transformations, many recent protection methods explicitly evaluate robustness under such operations to verify that the embedded perturbations remain effective after post-processing. 
% These transformation-based evaluations have therefore become an essential component of robustness assessment for perturbation-based protection methods.

Despite adopting different objectives and evaluation metrics, existing protocols share several common limitations. First, robustness is predominantly evaluated under isolated one-shot manipulations, whereas real-world images typically undergo multiple heterogeneous editing operations throughout their lifecycle. As a result, long-horizon robustness under sequential editing remains largely unexplored. Second, evaluations rely primarily on endpoint measurements after editing and therefore fail to characterize how protection robustness evolves throughout the editing process. Finally, the use of method-specific metrics prevents direct comparison across perturbation- and watermark-based protection paradigms. 
These limitations motivate the need for a unified robustness evaluation framework that not only enables fair comparison across heterogeneous protection paradigms but also characterizes robustness as an evolving process rather than a single endpoint.

==> round1/3_evaluation_protocol.tex <==
\section{PREEMPT}
\label{sec:method}

\subsection{Evaluation Pipeline}

To comprehensively simulate realistic post-deployment manipulations, we design a two-branch evaluation framework (see Fig.~\ref{fig:overview}) that evaluates protection robustness under both one-shot and long-horizon editing scenarios.  

\begin{figure*}[ht]
  \centering
    \includegraphics[width=\linewidth]{fig/framework.pdf}
    \caption{Overview of PREEMPT. Our framework evaluates proactive image protection methods under both one-shot and sequential editing scenarios. One-shot evaluation includes image-transformation-based edits and semantic edits, while sequential evaluation considers both homogeneous and heterogeneous edit chains to simulate realistic multi-step manipulations.}
    \label{fig:overview}  
\end{figure*}

\noindent\textbf{One-Shot Edit.} 
PREEMPT first evaluates robustness under isolated editing operations. One-shot evaluation consists of two complementary categories: \emph{Image-Transformation-based} and \emph{Semantic Edits}. Image Transformations simulate common pixel-level image processing operations encountered after image release, whereas semantic edits  evaluate robustness against content-level modifications generated by modern image editing models.

Transformation-based edits include commonly used image manipulations such as Gaussian blur, JPEG compression, crop-and-resize, horizontal flipping, and brightness/contrast adjustment. 
% Together, these operations represent typical post-processing encountered during image sharing and distribution.


% In addition to global transformations, we further consider semantic edits that modify local visual attributes while preserving the overall image structure. The semantic editing pipeline consists of three stages.

% First, following prior work~\cite{huang2018learning, joshi2026dota, foteinopoulou2026training}, we define the semantic editing space as $C=\{\text{Content}, \text{Attribute}, \text{Style}, \text{Spatial}\}$. Specifically, content edits modify object identity or semantic content; attribute edits adjust visual properties such as color, illumination, texture, or appearance; style edits alter artistic style or rendering medium; and spatial edits manipulate geometry, pose, or viewpoint. 

% Second, we employ a Large Language Model (LLM) to automatically generate editing prompts for each semantic category. Given an input image, the LLM first analyzes the visual scene and identifies the semantic domain and intended manipulation, and then produces category-specific editing instructions. To ensure prompt quality, we impose several constraints: edits should be realistic, visually grounded in the original image, diverse across semantic dimensions, and non-redundant. 

% Finally, the generated prompts are executed using state-of-the-art image editing models, including Stable Diffusion and InstructPix2Pix, to produce single-step semantic edits. Since the primary objective of proactive image protection methods is to interfere with downstream generation and customization processes, e.g., by degrading editing quality or preventing concept personalization, semantic edits provide a realistic and meaningful setting for evaluating their robustness.

Semantic edits are organized into four categories: Content, Attribute, Style, and Spatial, covering modifications to semantic content, visual attributes, artistic style, and spatial configuration, respectively. Category-specific editing prompts are automatically generated by a Large Language Model (LLM) and executed by state-of-the-art image editing models to produce one-shot semantic manipulations.

Together, transformation-based and semantic edits provide complementary evaluations of protection robustness under isolated editing scenarios.

\noindent\textbf{Sequential Edit.}
PREEMPT further evaluates robustness under long-horizon editing workflows. Sequential edit pipelines are composed of multiple editing operation combinations. From homogeneous to heterogeneous settings, we consider two complementary settings: \emph{Simple Chains} and \emph{Mixed Chains}.

Simple Chains consist of homogeneous semantic edits from a single semantic category, including content-only (C1), attribute-only (C2), style-only (C3), and spatial-only (C4). These chains isolate robustness degradation within individual semantic dimensions. 

Mixed Chains combine semantic edits with image-transformation-based operations to simulate practical editing workflows. Given a chain depth $d$, edit operations are sequentially sampled from the editing pool to generate diverse editing trajectories.

% Since semantic edits reconstruct image content and induce substantially larger changes than physical transformations, we focus on sequential semantic edits as the primary source of long-term modifications. The \emph{Simple Chain} consists of four homogeneous settings: content-only (C1), attribute-only (C2), style-only (C3), and spatial-only (C4), where each chain is composed of repeated edits from a single semantic category. These chains allow us to isolate the robustness degradation caused by each semantic dimension individually.

% We do not consider transformation-only chains, since consecutive physical transformations mainly accumulate as stronger low-level degradation and can often be approximated by a single transformation with adjusted parameters. In contrast, semantic edits introduce progressive content reconstruction and semantic drift, making their sequential effects inherently non-trivial. Therefore, we focus our homogeneous chains on semantic edits to isolate robustness degradation along different semantic dimensions.

% Nevertheless, real-world editing pipelines rarely consist of semantic edits alone. In practice, semantic modifications are often accompanied by platform-induced preprocessing or user-applied image transformations. Moreover, previous studies~\cite{} have shown that common transformations may already reduce protection effectiveness, while recent work~\cite{xue2024rethinking} show that diffusion-based reconstruction can further remove adversarial perturbations. Motivated by these observations, we introduce Mixed Chains (C5) that combine semantic edits with transformation-based operations, providing a more realistic and challenging evaluation setting for proactive image protection methods. Given a chain depth $d$, we randomly sample $d$ edit types from the editing pool and execute them sequentially, while allowing different execution orders. Randomization avoids order-specific bias and provides more diverse editing trajectories.

% By combining homogeneous semantic chains and heterogeneous mixed chains, PREEMPT evaluates protection robustness under both controlled semantic degradation and realistic multi-step editing scenarios. 
Figure~\ref{fig:qualitative} presents representative heterogeneous editing trajectories. Each trajectory combines transformation-based and semantic edits to simulate realistic editing workflows, motivating the need for a unified representation of robustness evolution. 
% Detailed implementation and experimental settings are presented in Sec.~\ref{sec:one_shot_results}.


\subsection{Protection Survival Representation}
% heterogeneous metrics → unified trajectory

Existing proactive protection paradigms rely on different robustness metrics. Perturbation-based methods typically measure semantic similarity between the edited and original images, whereas watermark-based methods evaluate message retrieval accuracy. Since these paradigm-specific metrics differ in both scale and interpretation, directly comparing robustness across protection methods is difficult.

To quantify robustness evolution in a unified manner, we define the normalized \emph{Protection Survival Ratio (PSR)} as:

\begin{equation}
\tilde{S}(d)=\frac{S(d)}{S(0)},
\label{eq:psr}
\end{equation}

where $S(d)$ denotes the robustness metric adopted by the corresponding protection paradigm after editing depth $d$, and $S(0)$ is the metric value of the protected-but-unedited image. For perturbation-based methods, $S(d)$ corresponds to semantic similarity, while for watermark-based methods it corresponds to message retrieval accuracy.

By normalizing with respect to the initial protected state, PSR removes differences in metric scales and expresses robustness as a relative survival trajectory over editing depth. This formulation enables robustness evolution to be analyzed consistently across heterogeneous protection paradigms while preserving the interpretation of each underlying evaluation metric.

Notably, PSR is designed to characterize the evolution of robustness rather than to unify the underlying task-specific metrics themselves. Consequently, trajectory-based analyses, such as survival curves and Protection AUC, can be applied consistently to different protection paradigms without altering their original evaluation objectives.


\subsection{Robustness Characterization}
% visual: curve, auc
To characterize long-horizon robustness, PREEMPT provides both a visual representation and a compact summary of protection survival trajectories.

\noindent\textbf{Protection Survival Curve.}
Given the normalized Protection Survival Ratio (PSR), robustness under sequential editing can be represented as a protection survival curve, \[ \{\tilde{S}(0), \tilde{S}(1), \ldots, \tilde{S}(D)\}, \] where each point corresponds to the normalized protection effectiveness after editing depth $d$. Starting from the normalized initial state ($S(0)=1$), the curve characterizes how protection effectiveness evolves throughout sequential editing. The resulting curve provides an intuitive representation of robustness evolution and facilitates comparison across protection methods and editing scenarios.

% Despite using different underlying metrics, both protection paradigms can be analyzed under the same trajectory-based framework, as shown in Fig.~\ref{fig:survival_curve}. For perturbation-based methods, homogeneous semantic chains exhibit a pronounced performance drop after the first edit, followed by a relatively stable plateau. In contrast, heterogeneous mixed chains show a more gradual degradation. Since transformation-based edits generally introduce limited semantic changes, their inclusion delays the overall collapse observed under purely semantic manipulations.

% The initial metric values reported in the legends additionally reveal the influence of protection itself before editing. For example, AdvDM and SDS(+) exhibit the lowest initial scores ($S(0)=0.87$), indicating that these methods introduce larger deviations from clean images. Nevertheless, compared with unprotected images, all perturbation-based methods exhibit varying degrees of protection effectiveness under subsequent edits.



% \begin{figure*}[htb]
%     \centering
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{fig/survival_heterogeneous_homogeneous_cx_perturbation_ip2p.pdf}
%         \caption{Perturbation-based methods.}
%         \label{fig:perturbation_curve}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{fig/survival_heterogeneous_homogeneous_cx_watermark_ip2p.pdf}
%         \caption{Watermark-based methods.}
%         \label{fig:watermark_cruve}
%     \end{subfigure}

%     \caption{Protection survival curves under homogeneous semantic chains and heterogeneous mixed chains. The legends report protection methods along with their initial preservation score $S(0)$, while the curves show the normalized Protection Survival Ratio defined in Eq.~\ref{Eq:PSR}. The dotted horizontal line denotes the half-life threshold ($S(d)/S(0)=0.5$). Perturbation-based methods exhibit a sharp degradation after the first edit, whereas watermark-based methods degrade more gradually and retain higher robustness throughout the editing process.
%     }
%     \label{fig:survival_curve}
% \end{figure*}

% For watermark-based methods, the trends are even more distinctive. VINE achieves better robustness under homogeneous semantic chains, whereas WAM becomes more resilient under heterogeneous mixed chains. This observation is consistent with the one-shot results presented earlier: VINE performs better under semantic edits, while WAM exhibits stronger robustness against transformation-based operations.

% Inspired by the notion of half-life in physics, we define the protection half-life as the editing depth at which the PSR falls below $0.5$, as illustrated by the horizontal reference line in Fig.~\ref{fig:survival_curve}:

% \begin{equation}
% d_{1/2}=\min_d \left\{\tilde S(d)\le0.5\right\}.
% \end{equation}

% As shown in Fig.~\ref{fig:perturbation_curve}, unprotected images typically maintain a half-life of four edits or more, whereas perturbation-based methods accelerate semantic degradation and often reach the half-life threshold after only one or two edits. In contrast, both watermarking methods remain above the threshold even after four editing steps, suggesting substantially stronger long-term robustness. The quantitative results of protection half-life are reported in supplementary material. 
\noindent\textbf{Protection AUC.}
While survival curves provide an intuitive visualization of robustness evolution, comparing a large number of trajectories across heterogeneous methods and scenarios can be cumbersome. We therefore summarize each trajectory using the area under the protection survival curve (AUC):

\begin{equation}
\mathrm{AUC}
=
\frac{1}{D}
\sum_{d=0}^{D-1}
\frac{\tilde{S}(d)+\tilde{S}(d+1)}{2},
\end{equation}

where $D$ denotes the maximum editing depth. Since $\tilde S(d)\in[0,1]$, the resulting AUC is also normalized to $[0,1]$, with larger values indicating stronger overall robustness throughout the editing process.


\begin{figure*}[th]
    \centering
    \includegraphics[width=\linewidth]{fig/trajectory_qualitative.pdf}
    \caption{Representative heterogeneous editing trajectories. Rows correspond to faces, artworks, and objects. Each trajectory consists of alternating transformation-based and semantic edits, illustrating the mixed editing workflow used throughout our sequential robustness evaluation.}
    \label{fig:qualitative}
\end{figure*}

==> round1/4_one_shot_results.tex <==
\section{One-shot Robustness}
\label{sec:one_shot_results}
% BUILD BASELINE
% We first investigate the robustness of protection methods under single-edit scenarios. Following the PREEMPT framework, we consider both image-transformation-based edits and semantic edits to establish baseline robustness before analyzing long-horizon degradation under sequential editing.
\subsection{Experimental Setup}

To demonstrate PREEMPT, we instantiate the framework using representative proactive image protection methods from both perturbation-based and watermark-based paradigms. Specifically, we evaluate four perturbation-based methods (PhotoGuard~\cite{salman2023raising}, Mist~\cite{liang2023mist}, AdvDM~\cite{liang2023adversarial}, and SDST~\cite{xue2023toward}) together with two recent watermarking methods (VINE~\cite{lu2024robust} and WAM~\cite{sander2025watermark}). These methods are selected to demonstrate the applicability of PREEMPT across various protection paradigms. To ensure fair comparison, all perturbation-based methods are generated using a standard perturbation budget ($\epsilon=12/255$) and 100 optimization steps. Clean images are additionally included as a no-protection baseline, denoted as \textit{None}.

% To quantify semantic changes under editing, we define a domain-specific semantic similarity metric. For biometric face images, semantic similarity is measured using ArcFace~\cite{deng2019arcface} identity cosine similarity. For artwork images, we adopt the cosine similarity between CSD~\cite{} style embeddings, while for object-centric images, we use DINOv2~\cite{} image feature similarity. Since these metrics are derived from different models and have different numerical ranges, we normalize their scores to a common scale for cross-domain comparison. A higher semantic similarity indicates that more semantic information from the original image is preserved after editing. Since successful image-based editing relies on transferring information from the source image, higher semantic similarity corresponds to more successful attacks and therefore weaker protection effectiveness.
Protection effectiveness is evaluated using the task-specific metrics corresponding to each protection paradigm. For perturbation-based methods, semantic similarity is measured using domain-specific feature representations: ArcFace~\cite{deng2019arcface} identity similarity for biometric faces, CSD~\cite{somepalli2024measuring} style embedding similarity for artworks, and DINOv2~\cite{oquab2023dinov2} feature similarity for natural scene images. The resulting scores are normalized to a common scale for cross-domain comparison. For watermark-based methods, robustness is measured by message retrieval bit accuracy using each method's official encoding and decoding pipeline. Following the original implementations, we embed the message ``Watermarked'' for VINE and ``WAMK'' for WAM according to their payload capacities.

% For watermarking methods, we evaluate two recent watermarking methods, VINE and WAM, each using their official watermark encoding and decoding pipelines. Due to the payload limitations of the respective methods, we embed the message 'Watermarked' for VINE and 'WAMK' for WAM. To assess robustness under editing, we use message retrieval bit accuracy as the evaluation metric, measuring whether the embedded information can still be successfully recovered after image modifications.

Image-transformation-based edits include Gaussian blur, JPEG compression, crop-and-resize, horizontal flipping, and brightness/contrast adjustment. These transformations~\cite{verdoliva2020media} represent typical post-processing encountered after image release. For semantic edits, four editing prompts are generated for each semantic category using GPT-4.1-mini~\cite{openai2023gpt4} and executed by two representative image editing models, Stable Diffusion v2.1~\cite{rombach2022high} and InstructPix2Pix~\cite{brooks2023instructpix2pix}. Since PREEMPT is independent of the underlying editing model, alternative editors can be incorporated without modifying the evaluation protocol.

The evaluation benchmark covers three representative visual domains: artwork images from WikiArt~\cite{artgan2018}, biometric face images from CelebA-HQ~\cite{liu2015deep, karras2018progressive}, and object-centric images from DreamBooth~\cite{ruiz2023dreambooth}. Curated subsets from these datasets are used throughout all experiments. Complete implementation details, parameter settings, and prompt templates are provided in the supplementary material.

% To instantiate the proposed evaluation framework, we adopt representative settings for each edit category. For transformation-based edits, we consider six commonly used operations, including Gaussian blur ($\sigma=2.0$), JPEG compression (quality factors of 50 and 70), crop-and-resize (cropping 85\% of the image area and resizing back to the original resolution), horizontal flipping, and brightness/contrast adjustment with a scaling factor of 1.5. These transformations are chosen to cover typical image processing operations and can be readily replaced by alternative parameter settings.
% For semantic edits, GPT-4.1-mini is employed to generate four editing prompts for each semantic category. The generated instructions are executed using two representative image editing models, Stable Diffusion v2.1 and InstructPix2Pix. Since our framework is independent of the underlying editing model, other editors can be incorporated in the same manner. 
% For sequential edits, the default editing depth is set to four in the main experiments, while additional depths are investigated in the ablation studies. The order of edits within each chain is randomly sampled using a fixed seed of 42 to ensure reproducibility. Unless otherwise specified, all random components in the editing pipeline use the same seed.


% Image-transformation-based edits include commonly used operations such as Gaussian blur, JPEG compression, crop-and-resize, horizontal flipping, and brightness/contrast adjustment. These operations are designed to simulate the automatic preprocessing pipelines employed by Online Social Networks (OSNs) when users upload images. Although the exact processing strategies vary across platforms, such transformations represent the most common and unavoidable manipulations encountered in practice. Previous studies~\cite{liu2023generating} have shown that adversarial perturbations are particularly fragile to these lossy operations introduced by OSNs. As a result, robustness to these transformations has been widely acknowledged as an important property of image protection methods, and many prior works~\cite{Tang_2026_CVPR, liu2024metacloak} include transformation robustness evaluations as part of their experimental studies. Rather than treating these tests as isolated ablations, our framework consolidates them into a unified and comprehensive evaluation protocol. Therefore, evaluating protection methods under these transformations is essential for assessing their practical robustness in real-world deployment scenarios.

% The semantic editing pipeline consists of three stages.
% First, following prior work~\cite{huang2018learning, joshi2026dota, foteinopoulou2026training}, we define the semantic editing space as $C=\{\text{Content}, \text{Attribute}, \text{Style}, \text{Spatial}\}$. Specifically, content edits modify object identity or semantic content; attribute edits adjust visual properties such as color, illumination, texture, or appearance; style edits alter artistic style or rendering medium; and spatial edits manipulate geometry, pose, or viewpoint. 
% Second, we employ a Large Language Model (LLM) to automatically generate editing prompts for each semantic category. Given an input image, the LLM first analyzes the visual scene and identifies the semantic domain and intended manipulation, and then produces category-specific editing instructions. To ensure prompt quality, we impose several constraints: edits should be realistic, visually grounded in the original image, diverse across semantic dimensions, and non-redundant. 
% Finally, the generated prompts are executed using state-of-the-art image editing models, including Stable Diffusion and InstructPix2Pix, to produce single-step semantic edits. Since the primary objective of proactive image protection methods is to interfere with downstream generation and customization processes, e.g., by degrading editing quality or preventing concept personalization, semantic edits provide a realistic and meaningful setting for evaluating their robustness.

\subsection{Image-Transformation-based edits}

Image-transformation-based edits evaluate protection robustness under common post-processing operations encountered during image sharing. The quantitative results for perturbation- and watermark-based methods are reported in Tab.~\ref{tab:per_l1_semantic_similarity} and Tab.~\ref{tab:wm_l1_retrieval_accuracy}, respectively.

\begin{table}[t]
\centering
\caption{Protection effectiveness of perturbation-based methods under one-shot image transformations. Metric: semantic similarity ($\downarrow$).}
\label{tab:per_l1_semantic_similarity}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc|c}
\toprule
Method & JPEG_{70} & JPEG_{50} & Bright.\&Contr. & Blur & Crop & Flip & Avg. \\
\midrule
\textit{None}  & 0.988 & 0.975 & 0.976 & 0.971 & 0.940 & 0.966 & 0.969 \\
AdvDM         & 0.874 & 0.872 & 0.869 & 0.880 & 0.824 & 0.858 & 0.863 \\
MIST          & 0.895 & 0.889 & 0.890 & 0.881 & 0.855 & 0.884 & 0.882 \\
PhotoGuard    & 0.895 & 0.890 & 0.890 & 0.880 & 0.856 & 0.885 & 0.883 \\
% SDS(+)         & 0.868 & 0.872 & 0.864 & 0.878 & 0.827 & 0.858 & 0.861 \\
% SDS(-)& 0.914 & 0.915 & 0.908 & 0.894 & 0.887 & 0.904 & 0.904 \\
SDST  & 0.899 & 0.896 & 0.896 & 0.884 & 0.865 & 0.890 & 0.888 \\
\bottomrule
\end{tabular}
}
\end{table}

% Table~\ref{transformation_perturbation_concept_similarity_ip2p} reports the semantic similarity after image-transformation-based edits. Higher similarity values indicate that more semantic information from the original image is preserved after editing, corresponding to weaker protection effectiveness.

% All perturbation methods consistently reduce semantic similarity relative to the unprotected baseline under all image transformations, indicating that protection effectiveness is largely preserved after common post-processing operations.

% Across different transformations, crop-and-resize leads to the lowest similarity values for almost all methods, implying that geometric modifications cause the largest degradation to semantic consistency. In comparison, JPEG compression and brightness/contrast adjustment have relatively minor influence. Overall, these results suggest that existing perturbation-based protections maintain a certain degree of robustness against common image transformations, while their effectiveness varies substantially across methods.



\begin{table}[t]
\centering
\caption{Protection effectiveness of watermark-based methods under one-shot image transformations. Metric: message retrieval accuracy ($\uparrow$).}
\label{tab:wm_l1_retrieval_accuracy}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc|c}
\toprule
Method & JPEG_{70} & JPEG_{50} & Bright.\&Contr. & Blur & Crop & Flip & Avg. \\
\midrule
VINE & 1.000 & 1.000 & 0.998 & 0.999 & 0.504 & 0.465 & 0.828 \\
WAM & 0.998 & 0.994 & 1.000 & 1.000 & 1.000 & 1.000 & 0.999 \\
\bottomrule
\end{tabular}
}
\end{table}


% Table~\ref{tab:wm_l1_retrieval_accuracy} reports message retrieval accuracy under common OSN-like image transformations. Overall, both watermarking methods maintain high decoding accuracy across most transformations, demonstrating strong robustness in practical deployment scenarios. WAM achieves nearly perfect retrieval performance under all evaluated operations, with an average accuracy of 0.999. VINE also remains highly robust to compression, blur, and brightness adjustments, but its performance drops significantly under crop-and-resize and horizontal flipping. This behavior can be attributed to the different embedding strategies of the two methods. VINE employs whole-image watermark embedding, enabling a larger payload of up to 12 characters, whereas WAM embeds information in localized regions and therefore supports only four characters. Consequently, geometric transformations that alter image layout have a stronger impact on VINE. Despite this trade-off, both methods successfully preserve watermark information under most OSN-like transformations, confirming the effectiveness of watermark-based protection.


Both protection paradigms remain largely robust under common image transformations. Compared with the unprotected baseline, perturbation-based methods consistently reduce semantic similarity across all evaluated transformations, while watermark-based methods maintain nearly perfect message retrieval accuracy under most operations. Crop-and-resize produces the largest performance degradation for both paradigms, whereas JPEG compression, Gaussian blur, and brightness/contrast adjustment have comparatively minor effects. These results indicate that routine post-processing alone is generally insufficient to invalidate existing proactive image protection methods.


\subsection{Semantic Edit}

% Although image transformations simulate common post-processing operations, they mainly introduce low-level pixel modifications. We next examine semantic edits, which directly alter image content and therefore pose a more challenging scenario for proactive protection.
Unlike image transformations, semantic edits directly modify image content and therefore provide a more challenging evaluation scenario. Unless otherwise specified, we report results obtained using InstructPix2Pix~\cite{brooks2023instructpix2pix} in the main paper, while the corresponding results using Stable Diffusion v2.1~\cite{rombach2022high} are provided in the supplementary material. The quantitative results are summarized in Tab.~\ref{tab:per_l2_semantic_similarity} and Tab.~\ref{tab:wm_l2_retrieval_accuracy}.


\begin{table}[t]
\centering
\caption{Protection effectiveness of perturbation-based methods under one-shot semantic edits. Metric: semantic similarity ($\downarrow$).}
\label{tab:per_l2_semantic_similarity}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc|c}
\toprule
Method & Content & Attribute & Style & Spatial & Average \\
\midrule
\textit{None} & 0.760 & 0.720 & 0.740 & 0.695 & 0.729 \\
AdvDM         & 0.267 & 0.234 & 0.331 & 0.249 & 0.270 \\
MIST          & 0.505 & 0.384 & 0.495 & 0.492 & 0.469 \\
PhotoGuard    & 0.490 & 0.372 & 0.486 & 0.462 & 0.453 \\
% SDS(+)         & 0.260 & 0.219 & 0.281 & 0.224 & 0.246 \\
% SDS(-)       & 0.216 & 0.202 & 0.389 & 0.306 & 0.278 \\
SDST  & 0.458 & 0.376 & 0.508 & 0.495 & 0.459 \\
\bottomrule
\end{tabular}
}
\end{table}

% Table~\ref{tab:l2_semantic_similarity_ip2p} quantifies the robustness results under one-shot semantic edits generated by InstructPix2Pix. The results are divided by each semantic edit type and the average value. Compared with clean images (0.729), all protection methods substantially reduce semantic consistency between the original and edited outputs, indicating that proactive protection remains effective under semantic manipulation. Semantic edits substantially reduce protection effectiveness compared with image transformations.
% Among all methods, SDS(+) achieves the strongest protection performance with the lowest average similarity (0.246), closely followed by AdvDM (0.270), while Mist, PhotoGuard, and Diff-Protect exhibit comparatively weaker resistance. Across edit categories, style edits consistently result in higher similarities than content and attribute edits, suggesting that stylistic modifications are more difficult to disrupt. In contrast, attribute edits generally produce the lowest similarities, implying that protection methods are particularly effective at suppressing localized semantic modifications. Moreover, different methods exhibit distinct sensitivities across edit categories, indicating that protection robustness is highly edit-dependent rather than uniformly distributed. Style Editing seems to be consistently the most resilient semantic edit category across protection methods. Results using Stable Diffusion 2.1 are provided in the Supplementary Material.

% Table~\ref{tab:wm_l2_retrieval_accuracy_ip2p} reports the message retrieval accuracy under one-shot semantic edits generated by InstructPix2Pix. Both watermarking methods maintain relatively high retrieval accuracy across all semantic edit categories, indicating that such edits do not completely destroy the embedded messages. VINE consistently outperforms WAM, achieving an average bit accuracy of 0.903 compared with 0.817 for WAM. Among different edit types, style edits lead to the largest performance degradation for both methods, with retrieval accuracy dropping to 0.850 for VINE and 0.733 for WAM. In contrast, content and spatial edits have comparatively smaller effects. These results suggest that modern watermarking methods exhibit strong robustness to one-shot semantic manipulations, although style transformations remain the most challenging scenario.

\begin{table}[t]
\centering
\caption{Protection effectiveness of watermark-based methods under one-shot semantic edits. Metric: message retrieval accuracy ($\uparrow$).}
\label{tab:wm_l2_retrieval_accuracy}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccc|c}
\toprule
Method & Content & Attribute & Style & Spatial & Average \\
\midrule
VINE & 0.945 & 0.899 & 0.850 & 0.917 & 0.903 \\
WAM  & 0.894 & 0.805 & 0.733 & 0.837 & 0.817 \\
\bottomrule
\end{tabular}
}
\end{table}

Compared with image transformations, semantic edits pose a substantially greater challenge to proactive image protection. Perturbation-based methods exhibit markedly lower protection effectiveness after a single semantic manipulation, while watermark-based methods also experience measurable retrieval degradation despite maintaining relatively high decoding accuracy. Across both protection paradigms, content-level modifications have a considerably stronger impact than low-level image transformations.

Nevertheless, these one-shot evaluations only measure protection effectiveness after an isolated edit and therefore provide static endpoint measurements. Whether such observations remain valid under realistic multi-step editing workflows is investigated in the next section.

==> round1/5_sequential_results.tex <==
\section{Long-Horizon Robustness}
\label{sec:sequential_result}

\subsection{Experimental Setup}
For long-horizon evaluation, we construct sequential editing chains with a default depth $d=4$ throughout the main paper. Results obtained using Stable Diffusion v2.1, together with additional long-horizon experiments, are presented in the supplementary material.

We consider two complementary sequential settings. Simple chains repeatedly apply semantic edits from a single category, enabling controlled evaluation of robustness evolution within individual semantic dimensions. Complex chains consist of heterogeneous edit sequences by combining semantic edits and image transformations, simulating practical multi-step editing workflows. Unless otherwise specified, edit operations are randomly sampled using a fixed seed of 42 to ensure reproducibility.

We do not consider transformation-only chains. Consecutive image transformations primarily accumulate low-level distortions and can often be approximated by a single transformation with adjusted parameters. In contrast, sequential semantic edits progressively reconstruct image content, resulting in substantially different robustness evolution. We therefore focus homogeneous chains on semantic edits while using heterogeneous chains to approximate realistic editing workflows.

\subsection{Robustness Evolution}
% Key Finding #1
% We plot the trajectories of homogeneous semantic chains and heterogeneous mixed chains in~\ref{fig:protection_survival_curve}. We find that robustness is a process, not a static endpoint. There're degradation dynamics for all the protection paradigms, from 0 to 4 depth. It continuous evoluate. One-shot editing evaluation cannot reveal this. Having established that robustness evolves over time, we next ask whether different protection paradigms evolve in the same way.

Figure~\ref{fig:protection_survival_curve} visualizes the evolution of protection robustness under sequential editing using the proposed PSR. Homogeneous semantic chains and heterogeneous mixed chains are shown separately to distinguish controlled semantic degradation from practical multi-step editing workflows.
Across both sequential settings, robustness evolves continuously with editing depth rather than collapsing after a single manipulation. All protection methods exhibit progressively decreasing PSR as additional edits are applied, indicating that robustness should be regarded as a dynamic property instead of a static endpoint.

This observation highlights an important limitation of conventional one-shot evaluation. Although measuring protection effectiveness after a single edit provides a useful snapshot of robustness, it does not reveal how protection evolves under realistic multi-step editing. Our results show that protection degrades progressively as edits accumulate, motivating trajectory-based analyses that capture robustness dynamics over the entire editing process.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{fig/Protection_survival_curve.pdf}
    \caption{Protection survival curves under homogeneous semantic chains (left) and heterogeneous mixed chains (right). Robustness evolves progressively with editing depth rather than remaining a static endpoint. The x-axis denotes the editing depth ($D=4$), and the y-axis shows the normalized Protection Survival Ratio (PSR). Solid lines indicate perturbation-based methods, and dashed lines indicate watermark-based methods. The legend reports each method together with its pre-edit effectiveness, $S(0)$).}
    \label{fig:protection_survival_curve}
\end{figure*}

\subsection{Paradigm-specific Evolution}
% Key Finding #2
Figure~\ref{fig:protection_family_survival_curve} compares the normalized robustness trajectories of perturbation- and watermark-based methods.Although both paradigms exhibit continuous robustness evolution under sequential editing, their evolution patterns differ substantially. Perturbation-based methods show a rapid change immediately after the first edit, followed by progressively diverging trajectories across methods. In contrast, watermark-based methods exhibit smoother and more consistent robustness evolution throughout the editing process. Sequential editing also increases the variability of robustness trajectories among perturbation-based methods, as reflected by the progressively wider spread across methods.
\begin{figure}[htb]
    \centering
    \includegraphics[width=.95\linewidth]{fig/Protection_family_survival_curve.pdf}
    \caption{Protection survival curves aggregated by protection paradigms. Shaded regions indicate the standard deviation across methods within each protection paradigm. Perturbation- and watermark-based methods exhibit distinct robustness evolution patterns under sequential editing.}
    \label{fig:protection_family_survival_curve}
\end{figure}

The observed difference is consistent with the different design objectives of the two protection paradigms. Perturbation-based methods protect images by disrupting downstream image generation, making their robustness closely coupled with semantic reconstruction during editing. Consequently, repeated semantic edits produce increasingly diverse robustness trajectories across different perturbation methods. In contrast, watermark-based methods aim to preserve an embedded signal for subsequent decoding. As long as sufficient watermark information survives each editing step, message retrieval remains relatively stable, leading to smoother robustness trajectories. These results indicate that robustness evolution is paradigm-dependent. Rather than enforcing a single robustness metric, PREEMPT accommodates paradigm-specific measurements within a unified trajectory-based evaluation framework, enabling consistent analysis and comparison of robustness evolution across different protection paradigms.

% Table~\ref{} summarizes these trajectories using Protection AUC. The consistent separation in AUC across both homogeneous and heterogeneous chains quantitatively confirms the distinct robustness evolution patterns observed in the survival curves.

% \begin{table}[htb]
% \centering
% \caption{Average protection survival AUC by protection paradigm. Higher AUC indicates stronger long-horizon robustness.}
% \label{tab:family_auc}
% \begin{tabular}{lc}
% \toprule
% Protection Paradigm & Average AUC \\
% \midrule
% Perturbation-based & 0.594 \\
% Watermark-based    & 0.849 \\
% \bottomrule
% \end{tabular}
% \end{table}

\subsection{Ranking Stability}
% Unexpected phenomenon

Ranking instability is primarily observed for perturbation-based methods. Since only two watermarking methods are evaluated and their relative ordering remains unchanged across editing depths, we focus the analysis on perturbation-based methods, where ranking changes are substantially more informative.

Figure~\ref{fig:rank_shift_heatmap} summarizes the average ranking change from one-shot ($d=1$) to long-horizon ($d=4$) evaluation. Positive values indicate that a method drops in ranking after sequential editing, whereas negative values indicate an improved ranking. Although all methods are evaluated under the same editing protocol, their relative rankings are not consistently preserved. For example, MIST, which ranks among the strongest methods after a single edit, consistently loses ranking under sequential evaluation, whereas AdvDM and SDST improve their relative positions across multiple edit settings.

\begin{figure}[th]
    \centering
    \includegraphics[width=\linewidth]{fig/rank_shift_heatmap_ip2p.pdf}
    \caption{Average ranking change from one-shot ($d=1$) to long-horizon ($d=4$) evaluation under homogeneous and heterogeneous edit chains. Positive values indicate that a method drops in ranking, while negative values indicate an improved ranking. The results show that method rankings obtained from one-shot evaluation are not consistently preserved under sequential editing.}
    \label{fig:rank_shift_heatmap}
\end{figure}

These observations suggest that one-shot robustness is not always predictive of long-horizon robustness. Methods exhibiting similar performance after a single edit may follow substantially different robustness trajectories under continued editing, eventually leading to different relative rankings. Consequently, evaluating proactive protection methods solely under one-shot settings may produce method rankings that do not generalize to realistic multi-step editing scenarios. 
Sequential evaluation therefore provides complementary information that cannot be inferred from one-shot robustness alone.

% To summarize the overall impact of these ranking changes, we further rank methods according to Protection AUC.

% \begin{table}[htb]
% \centering
% \caption{Protection survival AUC after sequential edits ($D=4$)}
% \label{tab:auc}
% \begin{tabular}{lcc}
% \toprule
% Method & Overall AUC & Rank\\
% \midrule
% MIST  & 0.616 & 2 \\
% PhotoGuard  & 0.616 & 2 \\
% AdvDM  & 0.524 & 1 \\
% SDST  & 0.620 & 3 \\
% \bottomrule
% \end{tabular}
% \end{table}

% Although MIST and PhotoGuard exhibit comparable one-shot robustness, their long-horizon AUC differs from AdvDM and SDST, resulting in a different overall method ordering. These observations further confirm that method selection depends on the evaluation protocol, highlighting the necessity of trajectory-aware robustness evaluation.

% \subsection{Trajectory Formation}
% Key Finding #3
\subsection{The Role of the First Semantic Edit}

Having established that protection robustness evolves throughout sequential editing, we next investigate what drives this evolution. Since heterogeneous edit chains consist of both image transformations and semantic edits, we group editing trajectories according to whether the first operation is a physical transformation or a semantic edit. 

Figure~\ref{fig:first_edit_type} compares the resulting robustness trajectories. When the first operation is an image transformation, protection robustness remains nearly unchanged after the first editing step, and the major robustness transition occurs only after subsequent semantic edits are introduced (see Fig.~\ref{fig:first_edit_type} (a)). In contrast, when the first operation is semantic, robustness exhibits an immediate transition after the first editing step, followed by substantially slower evolution throughout the remaining editing process (see Fig.~\ref{fig:first_edit_type} (b)). This contrast suggests that robustness evolution is more strongly associated with semantic edits than with low-level image transformations. Unlike image transformations, which mainly alter low-level image statistics while preserving semantic content, semantic edits explicitly reconstruct the image content, directly affecting the information that proactive protection methods seek to preserve or disrupt.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/sequential_perturbation_panels_ip2p.pdf}
    \caption{Robustness trajectories under heterogeneous edit chains grouped by the type of the first edit.
(a) Physical-first trajectories remain largely unchanged until the first semantic edit occurs.
(b) Semantic-first trajectories exhibit an immediate robustness transition followed by slower evolution.
Shaded regions denote the standard deviation across perturbation-based methods.
}
    \label{fig:first_edit_type}
\end{figure}

We further define the first-step contribution: 
\[ \alpha= \frac{\tilde{S}(0)-\tilde{S}(1)} {\tilde{S}(0)-\tilde{S}(D)}, \] 
which measures the fraction of the total robustness degradation occurring after the first editing step. The results are summarized in Tab.~\ref{tab:first-step-alpha}. Across homogeneous semantic chains, the first semantic edit accounts for approximately 63\%--93\% of the total degradation, indicating that most robustness change is concentrated in the initial semantic modification. In heterogeneous edit chains, however, this proportion consistently decreases to 44\%--52\%, suggesting robustness degrades more gradually across successive editing operations rather than being dominated by the first edit.

Taken together, these results indicate that semantic edits serve as the primary transition governing perturbation robustness, whereas image transformations largely preserve the existing robustness state until semantic reconstruction occurs. More importantly, they demonstrate that, under the evaluated editing scenarios, the evolution of protection robustness depends not only on editing depth but also on the composition of the editing sequence.

\begin{table}[t]
  \centering
  \caption{Contribution of the first editing step to the overall robustness evolution.
Higher $\alpha$ indicates that a larger proportion of robustness change occurs immediately after the first edit.
}
  \label{tab:first-step-alpha}
  \begin{tabular}{lcc}
    \toprule
    Method & Homo. $\alpha$ & Hetero. $\alpha$ \\
    \midrule
    PhotoGuard & 0.65 & 0.45 \\
    MIST       & 0.63 & 0.45 \\
    AdvDM      & 0.93 & 0.52 \\
    SDST       & 0.69 & 0.44 \\
    \bottomrule
  \end{tabular}
\end{table}



% \subsection{Overall comparison}

% To investigate the effect of edit composition, we compare homogeneous and heterogeneous editing chains. Homogeneous chains are composed of non-repeating edits from a single semantic category, whereas heterogeneous chains contain mixed edits spanning multiple semantic categories and image transformations.  Tables~\ref{tab:perturbation_chain_ip2p} and~\ref{tab:wm_chain_ip2p} summarize the final robustness after sequential editing.

% \begin{table}[ht]
% \centering
% \caption{Semantic similarity after sequential edits generated by InstructPix2Pix.}
% \label{tab:perturbation_chain_ip2p}
% \begin{tabular}{lccc}
% \toprule
% Method & Homo. & Hetero. & Avg. \\
% \midrule
% \textit{None}        & 0.492 & 0.630 & 0.561 \\
% AdvDM         & 0.274 & 0.397 & 0.336 \\
% MIST          & 0.275 & 0.503 & 0.389 \\
% PhotoGuard    & 0.279 & 0.506 & 0.393 \\
% SDS(+)         & 0.253 & 0.386 & 0.320 \\
% SDS(-)       & 0.233 & 0.449 & 0.341 \\
% SDST  & 0.300 & 0.510 & 0.405 \\


% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[ht]
% \centering
% \caption{Message retrieval accuracy after chain-of-simple edits using InstructPix2Pix.}
% \label{tab:wm_chain_ip2p}
% \begin{tabular}{lccc}
% \toprule
% Method & Homo. & Hetero. & Avg. \\
% \midrule
% VINE & 0.856 & 0.644 & 0.750 \\
% WAM  & 0.727 & 0.671 & 0.699 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \noindent\textbf{Perturbation-based Methods.}
% Compared with unprotected images, all protection methods continue to reduce semantic similarity after multiple editing steps, indicating that the protective effects are preserved to some extent even under sequential manipulation. Across most methods, heterogeneous chains lead to slightly higher similarities than homogeneous chains, suggesting that mixed edit compositions are generally more difficult to defend against. Nevertheless, the performance gap remains relatively small, implying that edit depth may have a greater influence on robustness than chain composition alone.


% \noindent\textbf{Watermark-based Methods.}
% Both watermarking methods maintain high message retrieval accuracy after four consecutive edits, with VINE consistently outperforming WAM. Since homogeneous chains already preserve most of the embedded messages, the results indicate that watermarking methods exhibit strong resistance to repeated semantic edits. Heterogeneous-chain results for watermarking are omitted because message decoding becomes unstable under mixed editing pipelines.



% \begin{table}[h]
% \centering
% \caption{Protection survival AUC after sequential edits ($D=4$)}
% \label{tab:auc}
% \begin{tabular}{lccc}
% \toprule
% Method & Homo. & Hetero. & Avg. \\
% \midrule
% \textit{None} & 0.691 & 0.791 & 0.741 \\
% SDST & 0.515 & 0.724 & 0.620 \\
% MIST & 0.508 & 0.725 & 0.616 \\
% PhotoGuard & 0.506 & 0.727 & 0.616 \\
% AdvDM & 0.417 & 0.631 & 0.524 \\
% \midrule
% \midrule
% VINE & 0.920 & 0.790 & 0.855 \\
% WAM & 0.831 & 0.853 & 0.842 \\
% \bottomrule
% \end{tabular}
% \end{table}

% The interpretation of AUC depends on the protection type: lower AUC indicates stronger perturbation-based protection, whereas higher AUC indicates stronger watermark robustness. Table~\ref{tab:auc}
% summarizes the overall robustness under sequential edits using Protection AUC with a maximum depth of $D=4$. The AUC values are consistent with the trends observed in the survival curves.

==> round1/6_additional_analysis.tex <==
\section{Additional Analysis}
\label{sec:additional_analysis}

To further validate the reasonableness of the proposed evaluation protocol, we conduct two additional analyses: (1) longer edit chains with depth $d=10$, and (2) mixed semantic edit chains.

\noindent\textbf{Sensitivity to Chain Length.} Our main experiments use edit chains with depth $d=4$, which provide a balance between evaluation cost and realistic editing scenarios. To address the concern that longer chains may exhibit substantially different behaviors, we further conduct an additional analysis with depth $d=10$. The longer heterogeneous chains consist of four semantic edits and six image-transformation-based edits. Note that this setting uses a different edit composition from the mixed chains in the main experiments and is not a direct extension of the $d=4$ setting.

As shown in Fig.~\ref{fig:curve_cx10_perturbation}, the degradation trends observed in the main experiments remain consistent under longer editing trajectories. Most perturbation-based methods continue to degrade gradually after the initial performance drop and reach the half-life threshold around depth 5--6. These results suggest that increasing the chain length mainly extends the degradation process rather than changing the overall conclusions. Therefore, the depth-4 setting used in the main experiments is sufficient to capture the primary robustness dynamics while keeping the evaluation cost manageable. Due to space limitations, the corresponding results for watermark-based methods are provided in the supplementary material.

\begin{figure}[htb]
    \centering
    \includegraphics[width=.95\linewidth]{fig/survival_curve_cx10_perturbation_ip2p.pdf}
    \caption{Protection survival curve of protection-based methods through 10-step heterogeneous edit chains.}
    \label{fig:curve_cx10_perturbation}
\end{figure}

\noindent\textbf{Mixed Semantic Chains.} 
To exclude the possibility that the observed degradation behavior is dominated by a particular semantic category, we further evaluate chains composed of mixed semantic edits. Specifically, each chain contains one edit from each semantic category following a fixed order: attribute, content, style, and spatial. The corresponding protection survival curves are shown in Fig.~\ref{fig:curve_c5}.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/survival_c5_perturbation_ip2p.pdf}
    \caption{Protection survival curves under mixed semantic edit chains.}
    \label{fig:curve_c5}
\end{figure}

Similar trends to those observed in the homogeneous semantic chains are consistently reproduced. In particular, the largest performance drop still occurs after the first edit, while subsequent edits contribute comparatively smaller degradation. This result indicates that the rapid initial performance loss is a general characteristic of semantic editing rather than an artifact of any specific semantic category.

==> round1/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Existing proactive protection methods typically follow evaluation settings adopted in prior work, and no standardized or comprehensive robustness benchmark currently exists. To address this gap, we propose PREEMPT, a protection robustness evaluation framework that covers both conventional one-shot editing scenarios and sequential editing scenarios that better reflect real-world manipulations. For sequential edits, we further introduce three complementary metrics: the Protection Survival Curve for visualizing degradation dynamics, Protection Half-Life for characterizing failure points, and Protection AUC for summarizing overall robustness. We hope PREEMPT can provide a common evaluation protocol for the community and facilitate the development of more robust and effective protection methods in the future.

In this paper, we present PREEMPT, a holistic evaluation framework for assessing the robustness of proactive image protection methods under realistic editing scenarios. 
% Unlike existing evaluations that primarily focus on isolated one-shot edits, we evaluate protection robustness under both one-shot and long-horizon editing scenarios. To enable consistent robustness analysis across various protection paradigms, we further introduced the Protection Survival Ratio, Curve, and AUC as unified robustness metrics. 
Rather than attempting to enumerate all possible editing chains, PREEMPT evaluates robustness through representative one-shot and sequential editing scenarios that provide a practical and reproducible evaluation protocol.
We introduce unified trajectory-based metrics, including the Protection Survival Ratio, Protection Survival Curve, and Protection AUC, to characterize robustness evolution across different protection paradigms.
% Extensive experiments on both perturbation- and watermark-based protection methods reveal several findings that are not observable under conventional one-shot evaluation. Protection robustness evolves continuously throughout sequential editing, different protection paradigms exhibit distinct evolution patterns, method rankings obtained from one-shot evaluation do not necessarily generalize to long-horizon scenarios, and semantic edits play a dominant role in shaping robustness evolution.
Beyond evaluating robustness, PREEMPT reveals three key insights. First, robustness evolves differently across protection paradigms. Second, similar one-shot robustness does not necessarily imply comparable long-horizon robustness, as methods may follow substantially different degradation trajectories under sequential editing. Third, robustness degradation is largely concentrated in the initial semantic edit, highlighting its dominant role in long-horizon robustness evolution. Together, these insights suggest that future protection methods should optimize robustness over the entire editing trajectory rather than at a single operating point. We hope PREEMPT serves as a foundation for future research on proactive image protection.


==> round2/6_additional_analysis.tex <==
\section{Additional Analysis}
\label{sec:additional_analysis}

To further validate the reasonableness of the proposed evaluation protocol, we conduct two additional analyses: (1) longer edit chains with depth $d=10$, and (2) mixed semantic edit chains.

\noindent\textbf{Sensitivity to Chain Length.} Our main experiments use edit chains with depth $d=4$, which provide a balance between evaluation cost and realistic editing scenarios. To address the concern that longer chains may exhibit substantially different behaviors, we further conduct an additional analysis with depth $d=10$. The longer heterogeneous chains consist of four semantic edits and six image-transformation-based edits. Note that this setting uses a different edit composition from the mixed chains in the main experiments and is not a direct extension of the $d=4$ setting.

As shown in Fig.~\ref{fig:curve_cx10_perturbation}, the degradation trends observed in the main experiments remain consistent under longer editing trajectories. Most perturbation-based methods continue to degrade gradually after the initial performance drop and reach the half-life threshold around depth 5--6. These results suggest that increasing the chain length mainly extends the degradation process rather than changing the overall conclusions. Therefore, the depth-4 setting used in the main experiments is sufficient to capture the primary robustness dynamics while keeping the evaluation cost manageable. Due to space limitations, the corresponding results for watermark-based methods are provided in the supplementary material.

\begin{figure}[htb]
    \centering
    \includegraphics[width=.95\linewidth]{fig/survival_curve_cx10_perturbation_ip2p.pdf}
    \caption{Protection survival curve of protection-based methods through 10-step heterogeneous edit chains.}
    \label{fig:curve_cx10_perturbation}
\end{figure}

\noindent\textbf{Mixed Semantic Chains.} 
To exclude the possibility that the observed degradation behavior is dominated by a particular semantic category, we further evaluate chains composed of mixed semantic edits. Specifically, each chain contains one edit from each semantic category following a fixed order: attribute, content, style, and spatial. The corresponding protection survival curves are shown in Fig.~\ref{fig:curve_c5}.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/survival_c5_perturbation_ip2p.pdf}
    \caption{Protection survival curves under mixed semantic edit chains.}
    \label{fig:curve_c5}
\end{figure}

Similar trends to those observed in the homogeneous semantic chains are consistently reproduced. In particular, the largest performance drop still occurs after the first edit, while subsequent edits contribute comparatively smaller degradation. This result indicates that the rapid initial performance loss is a general characteristic of semantic editing rather than an artifact of any specific semantic category.
